Explainable Decision Making with Lean and Argumentative Explanations

It is widely acknowledged that transparency of automated decision making is crucial for deployability of intelligent systems, and explaining the reasons why some decisions are "good" and some are not is a way to achieving this transparency. We consider two variants of decision making, where "good" decisions amount to alternatives (i) meeting "most" goals, and (ii) meeting "most preferred" goals. We then define, for each variant and notion of "goodness" (corresponding to a number of existing notions in the literature), explanations in two formats, for justifying the selection of an alternative to audiences with differing needs and competences: lean explanations, in terms of goals satisfied and, for some notions of "goodness", alternative decisions, and argumentative explanations, reflecting the decision process leading to the selection, while corresponding to the lean explanations. To define argumentative explanations, we use assumption-based argumentation (ABA), a well-known form of structured argumentation. Specifically, we define ABA frameworks such that "good" decisions are admissible ABA arguments and draw argumentative explanations from dispute trees sanctioning this admissibility. Finally, we instantiate our overall framework for explainable decision-making to accommodate connections between goals and decisions in terms of decision graphs incorporating defeasible and non-defeasible information.

==> background_preliminary.tex <==
\section{Introduction}
\label{sec:intro}

Decision making can be understood as a process of selecting ``good''
{\em decisions} amongst several alternatives, e.g. using {\em decision
  criteria}, based on relevant information available to the decision
maker, and a representation of this information.  

Argumentation-based decision making has attracted a considerable
amount of research interest over the years (e.g. see
\cite{Fox93,Nawwab08,Amgoud09,Fox10,Muller12}). Argumentation-based
decision making is a form of {\em qualitative decision theory}
\cite{Doyle99}, understood as an alternative to classical 
\emph{quantitative decision theory} \cite{French86} when a decision
problem cannot be easily formulated in standard decision-theoretic
terms using decision tables, utility functions and probability
distributions. In decision-theoretic terms, argumentation can be used
to compute a utility function which is too complex to be given a
simple analytical expression in closed form, and/or when a transparent
justification of decisions is beneficial.

Existing approaches to decision making using argumentation are
predominantly \emph{descriptive}, in that they are inspired by 
what people actually do and aim at justifying decisions by equipping
them with a \emph{transparent} explanation. For example,
\cite{Atkinson04} focuses on structuring arguments according to
well-defined argument schemes in order to justify and explain
decisions. In this work, we focus on {\em normative} decision 
theory, regulated by decision criteria fulfilling properties of
rationality. In other words, we first define the type of decision
making problems we want to solve and the decision criteria for solving
them, then we use argumentation as an alternative way to identify the
solutions.

We consider two representations to model information relevant to 
decision making. We start with {\em Abstract Decision Frameworks (ADFs)} 
consisting of {\em decisions}, {\em goals} and a {\em table} 
giving a {\em decisions-meeting-goals} relation. In the context of
ADFs, we study three decision criteria, {\em strong dominance,
  dominance}, and {\em weak dominance}, \respectively{} enforcing as
``good'' decisions meeting all goals, meeting all goals that are met
by any decision, and meeting goals not met by any other decision. 
Weak dominance corresponds to the well-known decision criterion of
Pareto optimality in decision theory \cite{Emmerich06} and 
strong dominance corresponds to selected decisions using the
conjunctive method in standard multi-attribute decision making
\cite{Yoon95}. We then introduce {\em preferences} over goals in ADFs,
and a corresponding a new decision criterion, that we call \pfrSet{},
enforcing as ``good'' decisions meeting the most preferred
goals. \pfrSet{} generalizes the lexicographic method in
multi-attribute decision making \cite{Yoon95}.

The second representation we consider is {\em decision graphs (DGs)}, a
graphical representation describing more complex relations between
decisions and goals. In a DG, a decision leads to {\em intermediate
  goals}, which in turn may lead to additional intermediate goals and
eventually to goals. With DGs, we have the ability to model {\em
  defeasibility} in decision making, by expressing, essentially, 
that ``a decision normally meets a goal, unless some
conditions hold''. 

For each of the proposed decision making frameworks (ADFs and DGs) and
respective decision criteria, we propose mappings into
assumption-based argumentation (ABA) frameworks
\cite{Bondarenko93,Bondarenko97,Dung09,Toni14} and prove that ``good''
decisions correspond to \emph{admissible arguments}, namely arguments
belonging to admissible sets, that are conflict-free and can defend
themselves against all attacks. In this way, we connect decision
making with argumentation, paving the way to explaining ``best''
decisions, e.g. following the approaches
of~\cite{Fan14-ECAI,Zhong14,Fan15-AAAI,Fan15-TAFA}. 

ABA is well-suited as a foundation for argumentation-based decision
making for a number of reasons. It is a general purpose argumentation
framework with several applications
(e.g. see~\cite{Dung09,Toni12,Toni14}), that has already proven useful
to support decision 
making~\cite{Matt09,Dung08,Fan13-CLIMA,Fan13-TAFA,Fan14-aamas,Carstens15}. It 
is a framework for structured argumentation~\cite{tutor}, allowing  
a fine-grained representation of the various components in a decision
model. At the same time, it is an instance of abstract
argumentation~\cite{Dung07,Toni12,Toni14} and it admits abstract 
argumentation as an instance~\cite{Toni12,Toni14}. Moreover, ABA is an
instance of ASPIC+~\cite{Prakken10}, another framework for structured
argumentation. ABA has strong theoretical
foundations~\cite{Bondarenko93,Bondarenko97}, with several formal
results readily available characterising the computational complexity
of various tasks in ABA~\cite{complexity:aij02,Dunne09-aba}. 
Another essential feature of ABA, for the purposes of this article, is
that it is equipped with provably correct computational mechanisms
\wrt{} several semantics~\cite{Dung06b,Dung07,aij12-XDDs}, which
includes {\em admissibility}. We rely upon aspects of these
mechanisms, as well as their soundness, to prove our soundness results. 
Finally, preliminary work on explanation in
ABA~\cite{Fan14-ECAI,Zhong14,Fan15-AAAI,Fan15-TAFA} can be used as the
starting point for explaining decisions obtained argumentatively.

This article is organised as follows. We recap ABA in
Section~\ref{sec:bkg}. We define ADFs and (three forms of) dominance 
in Section~\ref{sec:adf}, where we also give formal correspondence
results between dominance and standard mechanisms in decision making.
We then model decision making with preferences over goals in ADFs in
Section~\ref{sec:Pre}. We introduce DGs and decision making therein,
with and without defeasible information, in Section~\ref{sec:dg}. We
review related work in Section~\ref{sec:relatedWork} and  conclude in
Section~\ref{sec:conclusion}.

This article builds upon and generalises existing prior work as follows.
{\bf ADD HOW IT BUILDS UPON/EXPANDS PREVIOUS WORK}
\cite{Fan13-CLIMA,Fan13-TAFA,Fan14-aamas,Carstens15}.

The proofs of the technical results are all in Appendix~\ref{sec:proof}.

\section{Background}
\label{sec:bkg}

Material in this section is mostly adapted from \cite{Toni14}. 
An \emph{ABA framework} is a tuple $\langle \mc{L,R,A,C}\rangle$
where  
\begin{itemize}
\item $\langle \mc{L,R}\rangle$ is a deductive system, with a
 {\em language}  $\mc{L}$ and a set of inference {\em rules}
 $\mc{R}$ of the form $\sent_0 \gets \sent_1,\ldots, \sent_m (m > 0)$
 or $\sent_0 \leftarrow$ with  $\sent_i \in \mc{L}$, for $i=0, \ldots,
 m$,

\item $\mc{A} \subseteq \mc{L}$ is a (non-empty) set, whose
 elements are referred to as {\em assumptions},

\item $\mc{C}$ is a total mapping from $\mc{A}$ into
 $2^{\mc{L}} - \{\{\}\}$, where each $c \in \mc{C}(\alpha)$
  is a {\em contrary} of $\alpha$.

\end{itemize}

Basically, ABA frameworks can be defined for any logic specified by
means of inference rules. Some of the sentences in the underlying
language are assumptions, and each such sentence can be
``contradicted'' by any of its contraries. The following example is a
simple illustration, with a set of propositions as language. 

\begin{example}
\label{ABAAFEXP}
Let $\lracF$ be as follows:

$\bullet$
$\mc{L} = \{a, b, c, p, q, r,s\}$
and 
$\mc{R} = \{p \la a, \quad q \la b,s,\quad r \la c,\quad  s\la \}$,

$\bullet$
$\mc{A} = \{a, b, c\}$,

$\bullet$
$\mc{C}(a) = \{q\}$, $\mc{C}(b) = \{p\}$,
  $\mc{C}(c) = \{r, q\}$. 
\end{example}
%
Given a rule $\sent_0 \gets \sent_1,\ldots,\sent_m$ or $\sent_0
\leftarrow$ in an ABA framework, $\sent_0$ is referred as the {\em
  head} and $\sent_1,\ldots,\sent_m$ or the empty sequence,
\respectively, as the {\em body} of the rule. ABA frameworks where no
assumption occurs as the head of a rule are %referred to as 
{\em
  flat}. As an illustration, the ABA framework in
Example~\ref{ABAAFEXP} is flat, as assumptions there only occur in the 
body of rules. In this article, all ABA frameworks will be
flat. Therefore, all remaining definitions in this section are
restricted to the case of flat ABA frameworks. 

In ABA, informally, arguments are deductions of claims supported by
sets of assumptions, and attacks against arguments are directed at the
assumptions in their supports, and are given by arguments with an
assumption's contrary as their claim. Formally, given an ABA framework
\lracF, a \FT{{\em deduction for $\sent \in \mc{L}$ supported by} $\sentset
\subseteq \mc{L}$} is a \FT{finite} tree with nodes labelled by sentences in
$\mc{L}$ or by $\tau$\footnote{The symbol $\tau$ is such that $ \tau
  \notin \mc{L}$. $\tau$ stands for ``true'' and intuitively
  represents the empty body of rules~\cite{Dung09}.}, such that 
\begin{enumerate}
\item the root is labelled by $\sent$
\item for every node $N$
\begin{itemize}
\item if $N$ is a leaf then $N$ is labelled either by a sentence in
  $\sentset$ or  by $\tau$;
\item if $N$ is not a leaf and $\sent_0$ is the label of $N$, then there
 is an inference rule $\sent_0 \gets \sent_1,...,\sent_m (m \ge 0)$
 and either $m = 0$ and the child of $N$ is $\tau$ or $m > 0$ and $N$
 has $m$ children, labelled by $\sent_1,...,\sent_m$ (\respectively) 
\end{itemize}
\item $\sentset$ is the set of all sentences labelling the leaf nodes.
\end{enumerate}
Then, an {\em argument for $\sent \in \mathcal{L}$ supported by $\asmset \subseteq \mathcal{A}$} is a deduction for  $\sent$  supported by $\asmset$.
We will use the shorthand $\argu{\asmset}{\sent}$ to denote an argument for
$\sent$ supported by $\asmset$. Given argument $\argu{\asmset}{\sent}$,
$\asmset$ is referred to as the {\em support} and $\sent$ as the {\em
  claim} of the argument. Figure~\ref{argEXPS} illustrates this notion
of argument \FT{for the ABA framework} in Example~\ref{ABAAFEXP}.

\begin{figure}[h]
\begin{scriptsize}
\[\xymatrix@1@=12pt{
p                  &&&&& q                           &&&&& r \\
	a \ar@{-}[u]           &&&& b\ar@{-}[ur]  &  &s\ar@{-}[ul]       &&&& c \ar@{-}[u]\\
		   &&&&           & &  \tau \ar@{-}[u]   &&&& \\
{\argu{\{a\}}{p}}  &&&&& {\argu{\{b\}}{q}} &&&&& {\argu{\{c\}}{r}} }\] 
\end{scriptsize}
\caption{Arguments in Example~\ref{ABAAFEXP}, as trees (at the top) and
  using the shorthand (at the bottom).}
\label{argEXPS}
\end{figure}

Argumentation frameworks in general are useful for resolving conflicts between 
information, as captured by arguments. Conflicts are typically
represented as \emph{attacks} between arguments~\cite{Dung95}. In ABA,
attacks are defined in terms of the notion of contrary of assumptions,
as follows\FT{, given an ABA framework
\lracF}:

\begin{itemize}
\item an argument $\asmset_1 \vdash \sent_1$ attacks an argument
  $\asmset_2 \vdash \sent_2$ \ifaf{} the claim $\sent_1$ of the first argument
  is a contrary of one of the assumptions in the support $\asmset_2$
  of the second argument (i.e. $\exists \alpha \in \asmset_2$ such that
  $\sent_1 \in \mc{C}(\alpha)$);
\end{itemize}
This notion of attack between arguments can be lifted up to 
sets of arguments and sets of assumptions, as follows:
\begin{itemize}
\item a set of arguments \argAs{} attacks a set of arguments \argBs{} if
 some argument in \argAs{} attacks some argument in \argBs;
\item a set of assumptions $\asmset_1$ attacks a set of assumptions
  $\asmset_2$ \ifaf{} an argument supported by a subset of
  $\asmset_1$ attacks an argument supported by a subset of $\asmset_2$.
\end{itemize}
As an illustration, for the ABA framework in Example~\ref{ABAAFEXP},
\begin{itemize}
\item $\argu{\{a\}}{p}$ attacks $\argu{\{b\}}{q}$,
$\argu{\{b\}}{q}$ attacks $\argu{\{a\}}{p}$, $\argu{\{b\}}{q}$ attacks
$\argu{\{c\}}{r}$, and $\argu{\{c\}}{r}$ attacks $\argu{\{c\}}{r}$%FT. Also,
\item 
$\{\argu{\{a\}}{p}\}$ attacks $\{\argu{\{b\}}{q},\argu{\{c\}}{r}\}$ %FT and 
\item 
\{$a$\} attacks \{$b$\}, \{$b$\} attacks \{$a,c$\}, \{$b$\}
attacks \{$c$\}, and \{$c$\} attacks any set of assumptions containing $c$.
\end{itemize}

With argument and attack defined, all argumentation semantics
defined for abstract argumentation \cite{Dung95} can be applied in \FT{(flat)}
ABA. These semantics can be defined for assumptions, as in 
\cite{Bondarenko93,Bondarenko97}, or, equivalently, for
arguments~\cite{Dung07,Toni14}. In this article, given an ABA framework
$AF=\lracF$, we will use the following notions of admissibility for
sets of assumptions and for individual arguments: 
\begin{itemize}
\item 
\emph{a set of assumptions is admissible} (in $AF$) \ifaf{} it
does not attack itself and it attacks all $\asmset \subseteq \mc{A}$
that attack it;  

\item 
\emph{an argument $\argu{\asmset}{\sent}$ is admissible (in $AF$)
  supported by $\asmset'\subseteq \mc{A}$} \ifaf{} $\asmset \subseteq
\asmset'$ and $\asmset'$ is admissible (in $AF$).

\end{itemize}
As an illustration, for the ABA framework in Example~\ref{ABAAFEXP},
\begin{itemize}
\item the
sets of assumptions $\{a\}$, $\{b\}$, $\{\}$ are all admissible
(and no other set of assumptions is admissible); 

\item arguments $\argu{\{a\}}{p}$,  $\argu{\{b\}}{q}$, $\argu{\{a\}}{a}$, $\argu{\{b\}}{b}$
are all admissible (and no other argument is admissible).
\end{itemize}

\section{\FT{Preliminaries}}
\label{pre}

\FT{In the remainder of this section, unless specified otherwise, we will
assume as given a generic ABA framework 
$\lracF$.}

We will use variants of the {\em abstract dispute trees} of \cite{Dung06b} to
%FT prove some of our results later
provide explanations for recommended decisions. 
%
An \emph{abstract dispute tree}
for an argument \argA{} is a (possibly
infinite) tree \atree{} such that:\footnote{Here, $a$ stands for
  'abstract'. Also, \FT{`proponent' and `opponent' should be seen as roles/fictitious
  participants in a debate rather than actual agents.}} 

\begin{enumerate}
\item every node of \atree{} holds an argument $\argB$ 
	and is labelled by either {\em proponent} (P) or {\em opponent} (O),
  but not both, denoted by $L: \argB$, for $L \in \{$P,O$\}$;  
\item the root of \atree{} is a \pro{} node holding $\argA$;
\item for every \pro{} node $N$ holding an argument $\argB$, and
 for every argument $\tt C$ that attacks $\argB$, there
 exists a child of $N$, which is an \opp{} node holding $\tt C$;
\item for every \opp{} node $N$ holding an argument $\tt B$, there
 exists %FTdel exactly 
		\emph{at most}\footnote{\FT{In the original definition of abstract dispute tree~\cite{Dung06b}, every \opp{} node is required to have \emph{exactly} one child. We incorporate this requirement into the definition of \emph{admissible} dispute tree given later, so that our notion of admissible abstract dispute tree and the admissible abstract dispute trees of ~\cite{Dung06b} coincide.}} one child of $N$ which is a \pro{} node holding an argument
 which attacks some assumption $\alpha$ 
 in the support of $\tt B$;\footnote{An argument attacks an assumption
		if the argument supports a contrary of the assumption.}  \FT{if $N$ has a child attacking $\alpha$, then} $\alpha$ 
		is said to be the {\em culprit} in $\tt B$; 
\item there are no other nodes in \atree{} except those given by 1-4
 above.
\end{enumerate}
The set of all assumptions in (the support of arguments held by) the
\pro{} nodes in \atree{} is called the {\em defence set} of
\atree. 

Abstract dispute trees can be used as the basis for 
computing various argumentation semantics, including the admissibility semantics, as follows\del{,
given an ABA framework $AF$}:

\begin{itemize}
\item  
	\FT{Let an} abstract dispute tree \atree{} \FT{be} {\em admissible} \ifaf{} 
		each \opp{} node has {\em exactly} one child and no
culprit in the argument of an \opp{} node in \atree{} belongs to
the defence set of \atree. 
		\item The defence set of an admissible abstract
			dispute tree \del{for an argument $\argA$ (in $AF$)} is admissible (Theorem
		5.1 in \cite{Dung06b}), and thus \FT{the root node of an admissible dispute tree} \del{as well as the sentence in
		the root node of $\argA$} is admissible\del{ (in $AF$)}. 
	\item If an argument $\argA$ \del{(in $AF$)} is admissible then there exists an admissible abstract
		dispute tree for $\argA$ \del{(in $AF$)} (Theorem
		5.1 in \cite{Dung06b}).
\end{itemize}

%\begin{example}
%\label{disputeTreeExp}
%
%(Continuation of Example~\ref{ABAAFEXP})
Figure~\ref{argEXPS-ADT} gives an example of an (infinite) admissible
	dispute tree, with (admissible) defence set $\{a\}$\FT{, for the ABA framework in Example~\ref{ABAAFEXP}}. 

Given an abstract dispute tree $\atree$, let $N,N'$ be two nodes in
$\atree$. We say that $N$ is {\em reachable} from $N'$ (in $\atree$)
\ifaf{} following conditions hold:
\begin{enumerate}
\item
  $N'$ is a child of $N$, or

\item
  there is a node $N_0$ in $\atree$ \st{} $N'$ is a child of $N_0$ and
  $N$ is reachable from $N_0$.  
\end{enumerate}
In other words, $N$ is reachable from $N'$ \ifaf{} $N$ is an ``ancestor
node'' of $N'$.
        
\begin{figure}%[h]
\begin{scriptsize}
\[\xymatrix@1@=14pt{
\pro: \argu{\{a\}}{p} & \\
\opp: \argu{\{b\}}{q}\ar[u] & \\
\pro: \argu{\{a\}}{p}\ar[u] & \\                   
\vdots & 
}
\] 
\end{scriptsize}
\caption{Admissible abstract dispute tree for
  %Example~\ref{disputeTreeExp}.
	\FT{the ABA framework in Example~\ref{ABAAFEXP}}}
\label{argEXPS-ADT}
\end{figure}
%\end{example}


\FT{We will use three variants of abstract dispute trees, given below.}

%\begin{definition}
%  Let $\atree$ be an abstract dispute trees for some non-admissible
%  argument $\argA$. Then $\atree$ is {\em maximum} \ifaf{} there is no
%  node $\anode{X}{\_}, X \in \{P,O\}$ that can be added to $\atree$ \st{}
%  the revised tree is an abstract dispute tree for $\argA$.
%\end{definition}
%
%\FT{? USE THE NOTION OF MAXIMAL DISPUTE TREE IN \cite{AA-CBR-KR16} INSTEAD: }
% == OK

%\begin{definition}
A \emph{maximal dispute tree} \cite{AA-CBR-KR16} for some argument
$\argA$ is an abstract dispute tree \atree{} for $\argA$ \st{} for all
opponent nodes $\opp: \argB$ in \atree{} that are leaf nodes there is
no argument $\tt C$ \st\ $\tt C$ attacks $\argB$. 
%\end{definition}

Note that admissible abstract dispute trees are maximal, but not all
maximal dispute trees are
admissible~\cite{AA-CBR-KR16}. Given an ABA framework \lracF{} with
%\begin{itemize}
%\item
  $\mc{R} = \{c \gets \}$,
%
%\item
  $\mc{A} = \{a, b\}$,
%
%\item
  $\mc{C}(a) = \{b\}$, $\mc{C}(b) = \{c\}$,
%\end{itemize}
Figure~\ref{fig:maximalTrees} shows two abstract dispute trees for the
argument $\argu{\{a\}}{a}$, the tree on the left-hand side is maximal
whereas the one on the right-hand side is not.

\begin{figure}
  \begin{scriptsize}
    \[\xymatrix@1@=12pt{
      \pro: \argu{\{a\}}{a}       &&&&&& \pro: \argu{\{a\}}{a} \\
      \opp: \argu{\{b\}}{b}\ar[u] &&&&&& \opp: \argu{\{b\}}{b} \ar[u] \\
      \pro: \argu{\{\}}{c}\ar[u]  &&&&&&  \\      
    }\]
  \end{scriptsize}
  \caption{Two abstract dispute trees for the argument
    $\argu{\{a\}}{a}$. The tree shown on the left-hand side is
    maximal; the tree on the right-hand side is not.}
  \label{fig:maximalTrees}  
\end{figure}

%\FT{....GIVE EXAMPLE...} 

%\FT{WE COULD ALSO DEFINE SEMI-CONCRETE TREES SO THAT THE OPPONENT NODES ARE ALSO MEPS, AND THEN DEFINE MAXIMAL DISPUTE TREES IN TERMS OF THOSE? MAY BE AN OVERKILL...}

\begin{definition}
  \label{dfn:LAandBE}
Given any abstract dispute tree $\atree$, let
$LA(\atree)$ denote the set $\{\asm|\anode{\_}{\argu{\asmset}{\_}}$ is
a leaf node in $\atree, \asm \in \asmset\}$ and $LO(\atree)$ denote the
set $\{N|N=\anode{O}{\_}$ is a leaf node in $\atree$$\}$.

\begin{itemize}
\item
  Let $\mc{AT}$ be the set of all admissible abstract dispute trees
  for some argument $\argA$. Then $\atree \in \mc{AT}$ is {\em
    \leastAsm{}} \ifaf{} there is no $\atree_0$ in $\mc{AT}$ \st{}
  $LA(\atree_0) \subset LA(\atree)$. 

  \FT{\leastAsm{} NOT THE BEST NAME, LET US THINK OF A BETTER ONE...}

\item 
  Let $\mc{MT}$ be the set of all maximal dispute trees for some
  non-admissible argument $\argA$. Then $\mtree \in \mc{MT}$ is {\em
    best effort} \ifaf{} there is no $\mtree_0$ in $\mc{MT}$ \st{}
  $LO(\mtree_0) \subset LO(\mtree)$. 
\end{itemize}
\end{definition}

Given an ABA framework \lracF{} with $\mc{R} = \{a \gets b; a \gets c;
c \gets\}$, $\mc{A} = \{b, p, q\}$, $\mc{C}(b) = \{z\}$, $\mc{C}(p) =
\{q\}$, $\mc{C}(q) = \{a\}$, Figure~\ref{fig:LA} shows two  
abstract dispute trees for $\argu{\{p\}}{p}$, the tree on the
left-hand side is \leastAsm, the tree on the right-hand side is not.

\begin{figure}
  \begin{scriptsize}
    \[\xymatrix@1@=12pt{
      \pro: \argu{\{p\}}{p}       &&&&&& \pro: \argu{\{p\}}{p} \\
      \opp: \argu{\{q\}}{q}\ar[u] &&&&&& \opp: \argu{\{q\}}{q} \ar[u] \\
      \pro: \argu{\{\}}{a}\ar[u]  &&&&&& \pro: \argu{\{b\}}{a}\ar[u] \\            
    }\]
  \end{scriptsize}
  \caption{Two abstract dispute trees for the argument
    $\argu{\{p\}}{p}$. The tree shown on the left-hand side is
    \leastAsm; the tree on the right-hand side is not.}
  \label{fig:LA}  
\end{figure}

Given an ABA framework \lracF{} with $\mc{R} = \{b \gets; d \gets; f
\gets\}$, $\mc{A} = \{a,c,e\}$, $\mc{C}(a)=\{b,c\}$,
$\mc{C}(c)=\{d,e\}$, $\mc{C}(e)=\{f\}$, Figure~\ref{fig:BE} shows two
abstract dispute trees for $\argu{\{a\}}{a}$, the tree on the
left-hand side is best effort, the tree on the right-hand side is
not.

\begin{figure}
  \begin{scriptsize}
    \[\xymatrix@1@=12pt{
                                  & \pro: \argu{\{a\}}{a}       &&&&                             & \pro: \argu{\{a\}}{a} \\
      \opp: \argu{\{\}}{b}\ar[ur] & \opp: \argu{\{c\}}{c}\ar[u] &&&& \opp: \argu{\{\}}{b}\ar[ur] & \opp: \argu{\{c\}}{c}\ar[u] \\
                                  & \pro: \argu{\{\}}{d}\ar[u]  &&&&                             & \pro: \argu{\{e\}}{e}\ar[u]  \\            
                                  &                             &&&&                             & \opp: \argu{\{\}}{f}\ar[u] 
    }\]
  \end{scriptsize}
  \caption{Two abstract dispute trees for the argument
    $\argu{\{a\}}{a}$. The tree shown on the left-hand side is
    best effort; the tree on the right-hand side is not.}
  \label{fig:BE}  
\end{figure}

\begin{comment}
We will also use a variant of the notion of \emph{concrete dispute tree} of \cite{Dung06b}. Whereas the original concrete dispute trees incorporate the process towards the construction of arguments as well as failed attempts to identify further opponent nodes, our variant of concrete dispute trees in this paper only focuses on the latter, as follows. First, as in~\cite{aij12-XDDs}, 
\begin{itemize}
	\item a \emph{potential argument for $\sent\in \mathcal{L}$ supported by $\asmset \subseteq \mathcal{A}$ given $\sentset \subseteq \mathcal{L}$}, denoted as $\pargu{\asmset}{\sent}{\sentset}$, is a deduction for $\sent$ supported by $\asmset \cup \sentset$.
\end{itemize}

We will make use of the following restricted type of potential argument:

\begin{itemize}
	\item 
		a \emph{maximally expanded potential argument for $\sent$} (\emph{mep-argument} in short) is a potential argument $\pargu{\asmset}{\sent}{\sentset}$ \FT{(with \emph{support} $\asmset$)} such that \FT{$\sentset \cap \mathcal{A}=\{\}$} and %$\sentset\neq\{\}$ and 
		for all $\othersent \in \sentset$ there exists no rule in $\mathcal R$ with head $\othersent$. 
\end{itemize}

\FT{Note that potential arguments (including, but not limited to, mep-arguments) of the form $\pargu{\asmset}{\sent}{\sentset}$ with $\sentset=\{\}$ are arguments.
For example, given the ABA framework in Example~\ref{ABAAFEXP}, all mep-arguments are arguments.}
The following example provides a further illustration of mep-arguments. 

\begin{example}
\label{semi-concreteDTs}
\label{meps}
Given $\lracF$ with:

$\bullet$
$\mc{L} = \{a, b, c, p, q, r,s\}$
and 
$\mc{R} = \{p \la a, \quad q \la b, \quad q \la s, \quad r \la c \}$,

$\bullet$
$\mc{A} = \{a, b, c\}$,

$\bullet$
$\mc{C}(a) = \{q\}$, $\mc{C}(b) = \{r\}$,
  $\mc{C}(c) = \{s\}$
	\\
	$\pargu{\{\}}{s}{\{s\}}$ and 
	$\pargu{\{\}}{s}{\{q\}}$ are mep-argument which are not arguments,
	whereas $\pargu{\{a\}}{p}{\{\}}$ is a mep-argument which is an argument (namely $\argu{\{a\}}{p}$).
\end{example}

\FT{Note that mep-arguments are not guaranteed to exist. For example,
  given an ABA framework with rules including $p \leftarrow p$
  \FAN{(and no other rule $p \gets \_$) ??}, no
  mep-argument for $p$ exists. It is easy to see that mep-arguments
  for any sentence are guaranteed to exist in \emph{p-acyclic} ABA
  frameworks (see~\cite{Dung06b} for the formal definition of this
  notion),  where rules such as $p \leftarrow p$ are disallowed.} 

A {\em semi-concrete} dispute tree is defined as an abstract dispute tree, but with opponent nodes holding mep-arguments instead of arguments. 


\FT{
\begin{definition}
A \emph{semi-concrete} dispute tree 
for an argument \argA{} 
	is a (possibly
infinite) tree \ctree{} such that:
%
\begin{enumerate}
\item every node of \ctree{} 
	is labelled by either {\em proponent} (P) or {\em opponent} (O);
	every \pro{} node holds an argument, and every \opp{} node holds a mep-argument;
		a node holding an argument/mep-argument $\argB$ 
		is denoted by $L: \argB$, for $L \in \{$P,O$\}$;  
\item the root of \ctree{} is a \pro{} node holding $\argA$;
\item for every \pro{} node $N$ holding an argument $\argB$, and
 for every mep-argument $\tt C$ that attacks $\argB$, there
 exists a child of $N$, which is an \opp{} node holding $\tt C$;
\item for every \opp{} node $N$ holding a mep-argument $\tt B$, there
 exists \emph{at most} one child of $N$ which is a \pro{} node holding an argument
 which attacks some assumption $\alpha$ 
 in the support of $\tt B$; if $N$ has a child attacking $\alpha$, then
		$\alpha$ is said to be the {\em culprit} in $\tt B$; 
\item there are no other nodes in \ctree{} except those given by 1-4
 above.
\end{enumerate}
The set of all assumptions in (the support of arguments held by) the
\pro{} nodes in \ctree{} is called the {\em defence set} of
\ctree. 
\end{definition}
}

Given the ABA framework in Example~\ref{ABAAFEXP}, where all mep-arguments are arguments,  semi-concrete dispute trees are abstract dispute trees. 
	\FT{Figure~\ref{semi-concreteDTs} shows a semi-concrete dispute tree $\ctree$ (left) and an abstract dispute tree $\atree$ (right) for $\argu{\{a\}}{p}$,  given the ABA framework in Example~\ref{meps}. Note that \atree\ can be obtained from \ctree\ by deleting all mep-arguments that are not arguments.}

\begin{figure}%[h]
\begin{scriptsize}
\[\xymatrix@1@=14pt{
	&\pro: \argu{\{a\}}{p}&  && &\pro: \argu{\{a\}}{p} \\
	\opp: \argu{\{b\}}{q}\ar[ur] & & \opp: \pargu{\{\}}{q}{\{s\}}\ar[ul] & && \opp: \argu{\{b\}}{q}\ar[u]\\
	\pro: \argu{\{c\}}{r}\ar[u] & & && & \pro: \argu{\{c\}}{r}\ar[u]
	\\
	\opp: \pargu{\{\}}{s}{\{s\}}\ar[u] & &\\                   
}
\] 
\end{scriptsize}
	\caption{%Admissible 
		Semi-concrete dispute tree (left) and %admissible 
		abstract dispute tree (right) for
	Example~\ref{semi-concreteDTs}.
\label{semiCDT}
	}
\end{figure}

\FT{
\begin{definition}
	A semi-concrete dispute tree $\ctree$ is \emph{admissible} \ifaf\ 
each \opp{} node that holds an argument has exactly one
child and no culprit in the argument of an \opp{} node in $\ctree$ belongs to the
defence set of $\ctree$.
\end{definition}
}

\FT{It is easy to see that a semi-concrete dispute trees is admissible \ifaf\ the abstract dispute tree obtained by pruning all nodes holding mep-arguments is admissible. Therefore, the defence set of a semi-concrete dispute tree for some argument $\argA$ is admissible and $\argA$ is admissible, and if an argument $\argA$ is admissible then 
there exists a semi-concrete dispute tree for $\argA$.
}


\FT{IS THERE A LINK BETWEEN THE SEMI-CONCRETE TREES AND MAXIMAL/BEST EFFORT/LEAST ASSUMPTION?}


\FTb{
\begin{itemize}
	\item if admissible semi-concrete is admissible dispute tree then it is least assumption admissible too (but not vice versa)
\end{itemize}
}
\end{comment}

